Data augmentation and explainability for bias discovery and mitigation in deep learning

This dissertation explores the impact of bias in deep neural networks and presents methods for reducing its influence on model performance. The first part begins by categorizing and describing potential sources of bias and errors in data and models, with a particular focus on bias in machine learning pipelines. The next chapter outlines a taxonomy and methods of Explainable AI as a way to justify predictions and control and improve the model. Then, as an example of a laborious manual data inspection and bias discovery process, a skin lesion dataset is manually examined. A Global Explanation for the Bias Identification method is proposed as an alternative semi-automatic approach to manual data exploration for discovering potential biases in data. Relevant numerical methods and metrics are discussed for assessing the effects of the identified biases on the model. Whereas identifying errors and bias is critical, improving the model and reducing the number of flaws in the future is an absolute priority. Hence, the second part of the thesis focuses on mitigating the influence of bias on ML models. Three approaches are proposed and discussed: Style Transfer Data Augmentation, Targeted Data Augmentations, and Attribution Feedback. Style Transfer Data Augmentation aims to address shape and texture bias by merging a style of a malignant lesion with a conflicting shape of a benign one. Targeted Data Augmentations randomly insert possible biases into all images in the dataset during the training, as a way to make the process random and, thus, destroy spurious correlations. Lastly, Attribution Feedback is used to fine-tune the model to improve its accuracy by eliminating obvious mistakes and teaching it to ignore insignificant input parts via an attribution loss. The goal of these approaches is to reduce the influence of bias on machine learning models, rather than eliminate it entirely.

==> Parts/Part1.tex <==

\part{XAI for discovering bias in data and models}

\lhead{\emph{Chapter 2: Bias in machine learning pipeline}}  % Set the left side page header to "Chapter 1"
\input{Chapters/2_Bias_in_ML} % Background Theory - Bias in data and models

\clearpage  %Start a new page
\lhead{\emph{Chapter 3: Explainable Artificial Intelligence}}  % Set the left side page header to "Chapter 1"
\input{Chapters/3_XAI} % Experimental Setup


\clearpage  %Start a new page
\lhead{\emph{Chapter 4: Identifying bias with manual data inspection}}  % Set the left side page header to "Chapter 1"
\input{Chapters/4_isic_bias} % Experimental Setup

\clearpage  %Start a new page
\lhead{\emph{Chapter 5: Identifying bias with global explanations}}  % Set the left side page header to "Chapter 1"
\input{Chapters/5_GEBI} % Experimental Setup



==> Parts/Part2.tex <==
\part{Mitigating bias in data and models}

% \clearpage  %Start a new page
% \lhead{\emph{Chapter 6: On bias mitigation: achievements, goals and perspectives}}  % Set the left side page header to "Chapter 1"
% \input{Chapters/6_bias_mitigation} % Experiment 1

\clearpage  %Start a new page
\lhead{\emph{Chapter 6: Mitigating shape and texture bias with data augmentation}}  % Set the left side page header to "Chapter 1"
\input{Chapters/7_NST} % Experiment 2
% side page header to "Chapter 1"

\clearpage  %Start a new page
\lhead{\emph{Chapter 7: Bias-targeted data augmentation}}  % Set the left 
\input{Chapters/8_bias_targeted_da} % Results and Discussion

\clearpage  %Start a new page
\lhead{\emph{Chapter 8: Debiasing effect of training with attribution feedback}}  % Set the left side page header to "Chapter 1"
\input{Chapters/9_attribution_feedback} % Conclusion


==> Preamble/Declaration.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Declaration{
\addtocontents{toc}{}  % Add a gap in the Contents, for aesthetics

I, the undersigned, agree that my PhD dissertation entitled: \textit{Data augmentation and explainability
for bias discovery and mitigation in deep learning} may be used for scientific or didactic purposes \footnote{Decree of Rector of Gdansk University of Technology No. 34/2009 of 9th November 2009, TUG archive instruction addendum No. 8.}.

\vfil\vfil\null
Signature:\\
\rule[1em]{25em}{0.5pt}  % This prints a line for the signature

Print Name: Agnieszka Mikołajczyk\\
\rule[1em]{25em}{0.5pt}  % This prints a line for the signature

Date:\\
\rule[1em]{25em}{0.5pt}  % This prints a line to write the date

\addtocontents{toc}{}

\vfil

\textbf{Declaration}

I, the undersigned, agree to include an electronic version of the above PhD dissertation in the open, institutional, digital repository of \textit{Gdańsk University of Technology, Pomeranian Digital Library}, and for it to be submitted to the processes of verification and protection against misappropriation of authorship.

\vfil\vfil\null
Signature:\\
\rule[1em]{25em}{0.5pt}  % This prints a line for the signature

Print Name: Agnieszka Mikołajczyk\\
\rule[1em]{25em}{0.5pt}  % This prints a line for the signature

Date:\\
\rule[1em]{25em}{0.5pt}  % This prints a line to write the date

}


==> Preamble/Declaration_publications.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Declarationpublication{
\addtocontents{toc}{}  % Add a gap in the Contents, for aesthetics
TO-DO

\emph{This declaration is to be included in a `thesis including published works'. You must provide details of all publications included in your thesis in the section below. If you have not completed a thesis including published works.}

\emph{Please ensure your thesis meets the \href{https://www.monash.edu/graduate- esearch/examination/publication}{thesis including published works requirements}. Some faculties vary requirements in terms of the number of papers required, status of papers
and other criteria. These faculty specific requirements can also be found at the above link.}

\emph{Please remove the above section and include a standard thesis declaration.}

I hereby declare that this thesis contains no material which has been accepted for the award of any other degree or diploma at any university or equivalent institution and that, to the best of my knowledge and belief, this thesis contains no material previously published or written by another person, except where due reference is made in the text of the
thesis.

This thesis includes (\emph{insert number)} original papers published in peer reviewed journals and (\emph{insert number)} submitted publications. The core theme of the thesis is (\emph{insert theme}). The ideas, development and writing up of all the papers in the thesis were the principal responsibility of myself, the student, working within the
(\emph{insert name of academic unit}) under the  supervision of (\emph{insert name of supervisor}).

(The inclusion of co-authors reflects the fact that the work came from active collaboration between researchers and acknowledges input into
team-based research.) \emph{Remove this paragraph for theses with sole-authored work}

In the case of \emph{(insert chapter numbers}) my  contribution to the work involved the following:

\emph{(If this is a laboratory-based discipline, a paragraph outlining the assistance given during the experiments, the nature of the experiments and an attribution to the contributors could follow.})

Here should be the table!

I have / have not renumbered sections of submitted or published papers
in order to generate a consistent presentation within the thesis.

Student name:

Student signature: Date:

I hereby certify that the above declaration correctly reflects the
nature and extent of the student's and co-authors' contributions to this
work. In instances where I am not the responsible author I have
consulted with the responsible author to agree on the respective
contributions of the authors.

\textbf{Main Supervisor name: prof. Michał Grochowski}

\textbf{Main Supervisor signature:} \textbf{Date:}


}

==> Preamble/Preface.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
\Preface{

\addtocontents{toc}{}  % Add a gap \vspace{1em} in the Contents, if for aesthetics

Where applicable, the following information must be included in a preface:
\begin{itemize}
\item[\tiny{$\blacksquare$}] a description of work towards the thesis that was carried out in collaboration with others, indicating the nature and proportion of the contribution of others and in general terms the portions of the work which the student claims as original;
\item[\tiny{$\blacksquare$}] a description of work towards the thesis that has been submitted for other qualifications;
\item[\tiny{$\blacksquare$}] a description of work towards the thesis that was carried out prior to enrolment in the degree;
\item[\tiny{$\blacksquare$}] whether any third party editorial assistance was provided in preparation of
the thesis and whether the persons providing this assistance are knowledgeable in the academic discipline of the thesis;
\item[\tiny{$\blacksquare$}] the contributions of all persons involved in any multi-authored publications or
articles in preparation included in the thesis;
\item[\tiny{$\blacksquare$}] the publication status of all chapters presented in article format using the
descriptors below;
    \begin{itemize}
        \item Unpublished material not submitted for publication
        \item Submitted for publication to [publication name] on [date]
        \item In revision following peer review by [publication name]
        \item Accepted for publication by [publication name] on [date]
        \item Published by [publication name] on [date]
    \end{itemize}
\item[\tiny{$\blacksquare$}] an acknowledgement of all sources of funding, including grant identification
numbers where applicable and Australian Government Research Training Program Scholarships, including fee offset scholarships.
\end{itemize}

}

==> Preamble/Publications.tex <==
% https://www.monash.edu/graduate-research/examination/publication
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis
% https://www.monash.edu/rlo/graduate-research-writing/write-the-thesis/writing-the-thesis-chapters/structuring-a-long-text
% \Publicationslist{

\addtocontents{toc}{}  % Add a gap  \addtocontents{toc}{\vspace{1em}}  in the Contents, for aesthetics

Journal articles:

\begin{enumerate}
\item Mikołajczyk, A., Grochowski, M., and Kwasigroch, A. 2021. Towards explainable classifiers using the counterfactual approach-global explanations for discovering bias in data. Journal of Artificial Intelligence and Soft Computing Research, 11(1), p.51–67.
\item Klawikowska, Z., Mikołajczyk, A., and Grochowski, M. 2020. Explainable AI for Inspecting Adversarial Attacks on Deep Neural Networks. In International Conference on Artificial Intelligence and Soft Computing (pp. 134–146).
\item Mikołajczyk, A., and Grochowski, M. 2019. Style transfer-based image synthesis as an efficient regularization technique in deep learning. In 24th International Conference on Methods and Models in Automation and Robotics, arXiv:1905.10974.
\item Grochowski, M., Mikołajczyk, A., and Kwasigroch, A. 2019. Diagnosis of malignant melanoma by neural network ensemble-based system utilising hand-crafted skin lesion features. Metrology and Measurement Systems, 26(1), p.65–80.
\item Mikołajczyk, A., and Grochowski, M. 2018. Analiza istotno\'sci cech znamion skórnych dla celów diagnostyki czerniaka złośliwego. Zeszyty Naukowe Wydziału Elektrotechniki i Automatyki Politechniki Gdańskiej.
\item Grochowski, M., Kwasigroch, A., and Mikołajczyk, A. 2019. Selected Technical Issues of Deep Neural Networks for Image Classification Purposes. Bulletin of the Polish Academy of Sciences: Technical Sciences, 67(2), p.363–376.
% \item Grochowski, M., Wąsowicz, M., Mikołajczyk, A., Ficek, M., Kulka, M., Wróbel, M., and Jędrzejewska-Szczerska, M. 2019. Machine learning system for automated blood smear analysis. Metrology and Measurement Systems, 26(1), p.81–93.
% \item Mikolajczyk, A., Grochowski, M., and Kwasigroch, A. 2018. Optimal Selection of Input Features and an Acompanying Neural Network Structure for the Classification Purposes-Skin Lesions Case Study. In 2018 23rd International Conference on Methods & Models in Automation & Robotics (MMAR) (pp. 899–904).
\item Mikołajczyk, A., and Grochowski, M. 2018. Data augmentation for improving deep learning in image classification problem. In 2018 International Interdisciplinary PhD Workshop (IIPhDW) (pp. 117–122).
% \item Kwasigroch, A., Mikołajczyk, A., and Grochowski, M. 2017. Deep neural networks approach to skin lesions classification—A comparative analysis. In 2017 22nd International Conference on Methods and Models in Automation and Robotics (MMAR) (pp. 1069–1074).
% \item Wąsowicz, M., Grochowski, M., Kulka, M., Mikołajczyk, A., Ficek, M., Karpieńko, K., and Cićkiewicz, M. 2017. Computer aided detection of abnormal erythrocytes for analysis of the in vitro interactions of nanodiamonds with human blood. In The Second International Conference.
\item Kwasigroch, A., Mikołajczyk, A., and Grochowski, M. 2017. Deep convolutional neural networks as a decision support tool in medical problems–malignant melanoma case study. In Polish Control Conference (pp. 848–856).
\item Mikołajczyk, A., Kwasigroch, A., and Grochowski, M. 2017. Intelligent system supporting diagnosis of malignant melanoma. In Polish Control Conference (pp. 828–837).
\end{enumerate}

